SparseDC: Depth Completion from sparse and non-uniform inputs

We propose SparseDC, a model for Depth Completion of Sparse and non-uniform depth inputs. Unlike previous methods focusing on completing fixed distributions on benchmark datasets (e.g., NYU with 500 points, KITTI with 64 lines), SparseDC is specifically designed to handle depth maps with poor quality in real usage. The key contributions of SparseDC are two-fold. First, we design a simple strategy, called SFFM, to improve the robustness under sparse input by explicitly filling the unstable depth features with stable image features. Second, we propose a two-branch feature embedder to predict both the precise local geometry of regions with available depth values and accurate structures in regions with no depth. The key of the embedder is an uncertainty-based fusion module called UFFM to balance the local and long-term information extracted by CNNs and ViTs. Extensive indoor and outdoor experiments demonstrate the robustness of our framework when facing sparse and non-uniform input depths. The pre-trained model and code are available at https://github.com/WHU-USI3DV/SparseDC.

==> sec/i_intro_bk_lc.tex <==
\section{Introduction}
\label{sec:intro}
% 加引用
Acquiring dense and accurate depth is crucial in various fields, such as autonomous driving\cite{yurtsever2020survey,maurer2016autonomous}, 3D reconstruction\cite{geiger2011stereoscan,long2022pc2,pan2016dense}, scene understanding\cite{cordts2016cityscapes,li2009towards}, AR/VR\cite{yuen2011augmented,park2019literature}. Although the commonly used depth sensors, such as Microsoft Kinect\cite{zhang2012microsoft}, Intel RealSense\cite{keselman2017intel}, LIDAR\cite{atanacio2011lidar}, can obtain depth within their effective field of view, it is still a great challenge to obtain dense depth maps due to environment, equipment, and cost limitations. In recent years, depth completion, serving as a cost-effective means to achieve dense pixel-wise depth, has become a long-standing research endeavor that has captivated the attention of many researchers.

Despite achieving impressive performance on benchmark datasets\cite{nyu,kitti}, existing state-of-the-art methods\cite{wang2023lrru,youmin_completionformer_2023,yan_rignet_2022,zhou_bev_2023} often fall short in some challenging cases.
In contrast to the fixed data distribution of the benchmark dataset(e.g., NYU Depth\cite{nyu} with 500 points, Kitti\cite{kitti} with 64 lines), the inputs in real scenarios may be non-uniform and sparser. For example, researchers often employ depth sensors with lower resolutions (Velodyne HDL-16E LiDAR, VCSEL ToF sensors) to mitigate costs. In addition, environmental factors easily influence sensors, such as high-reflectivity objects and multipath effects resulting in uneven distribution of effective depth points. \textit{\textbf{Regrettably, mainstream methods primarily focus on the sparse-to-dense completion process without realizing the sparsity changes and the non-uniform distribution of depth points}}. Consequently, they are difficult to reconstruct the scene structure when the spatial pattern of the input significantly deviates from the distribution observed in the benchmark dataset during training, as illustrated in \cref{fig:teaser}
% Recent methods focused on stacking complex network architectures and designing sophisticated training strategies, 

% Depth completion aims to recover dense pixel-wise depths from sparse depth maps captured by sensors. In its early stages, previous depth completion methods heavily relied on prior scene knowledge, employing various planar assumptions to interpolate the sparse depth image. In recent years, with the rapid advancements in deep learning, learning-based approaches have emerged as more competitive alternatives, gradually dominating this field. As a pioneering work based on deep learning, Uhrig et al. proposed Sparsity Invariant CNN\cite{Sparsitycnn}, which directly maps sparse depths to dense depth maps using sparse convolution. 
% In contrast to the fixed data distribution of the benchmark dataset(e.g., NYU Depth with 500 points, Kitti with 64 lines), the inputs in real scenarios are non-uniform and sparser. For example, researchers often employ depth sensors with lower resolutions (Velodyne HDL-16E LiDAR, VCSEL ToF sensors) in real cases to mitigate costs. In addition, environmental factors easily influence sensors, such as high-reflectivity objects and multipath effects resulting in uneven distribution of effective depth points. \textit{\textbf{Regrettably, existing state-of-the-art methods primarily focus on the sparse-to-dense completion process without realizing the sparsity changes and the non-uniform distribution of depth points}}. Consequently, they are difficult to reconstruct the scene structure when the spatial pattern of the input significantly deviates from the distribution observed in the benchmark dataset during training, as illustrated in \cref{fig:teaser}.

To address this challenge, a naive solution is to simulate diverse spatial distributions during training, utilizing a large parameter model to enable the network to adapt to various scenarios. 
% However, designing an effective simulation strategy is highly challenging due to the inherent complexity of real environments. 
However, this augment-based solution easily leads to overfitting on the training set, and highly variable inputs make it difficult to extract stable features during training\cite{woo2023convnext,graham2017submanifold,spconv2022,Sparsitycnn}.
Furthermore, we observed when dealing with sparser cases, the nature of the task transitions from relying on local details to relying more heavily on global image semantics for a holistic scene understanding.
% which poses limitations of mainstream methods designed only for fixed distribution. 
To demonstrate this point, we conducted a simple experiment, where we selected ResNet-18\cite{resnet} and PvtV2-b1\cite{pvt, pvtv2} as two backbone networks; one is known for its ability to extract local features and capture fine-grained details, and the other focuses on capturing the overall scene context and leveraging global relationships between pixels. We used the NYU Depth V2\cite{nyu} to test, and recorded the final results of the two backbone networks separately. As illustrated in \cref{anaylse}, as the density of depth points decreases, the global scene information plays a more important role in depth completion. An intuitive explanation is that high-density depth points are sufficient to provide rich local context and detail for depth completion, while for low-density inputs, we need to understand the overall scene to fill large areas.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/analyse1.jpg}
    % \caption{\textbf{Pilot study results on NYU Depth V2 dataset}. The first row shows the quantitative analysis. The horizontal axis represents the number of effective depth points in each testing depth map. The vertical axis illustrates the number of testing depth maps for which the network outperforms the other in RMSE. The second row is the qualitative results. We visualize the difference in accuracy between different branches, the darker colors indicating more accurate depth predicted by PvtV2-b1.}
    \caption{\textbf{Pilot study results on NYU Depth V2 dataset}. The horizontal axis represents the number of effective depth points in each testing depth map. The vertical axis illustrates the number of testing depth maps for which the network outperforms the other in terms of RMSE.}
    \label{anaylse}
    \vspace{-1em}
\end{figure}
%Based on this observation, we propose a novel depth completion network framework named SparseDC. The key idea behind SparseDC is to \textit{\textbf{effectively leverage the complementary strengths of local details and global semantics to improve the robustness of depth completion in the presence of sparse and non-uniform inputs}}. The whole framework of SparseDC is illustrated in \cref{fig:overview}.  Firstly, we adopt a two-branch feature extraction structure, thus allowing the model to comprehend the holistic scene context while modeling intricate local scale details. Then, some studies proved that uneven input would cause feature fluctuations\cite{woo2023convnext,graham2017submanifold,spconv2022,Sparsitycnn}, making it difficult for our feature extractor to generalize to various spatial distributions of depth points. So, we design a \textit{Sparse Feature Filling Module} that uses immutable image features to fill the varying depth features, thereby improving the stability of the features extracted by different branches. Finally, the fusion of the extracted features plays a crucial role in SparseDC. To tackle this, we introduce an \textit{Uncertainty-Guided Feature Fusion Module(UFFM)}. The UFFM estimates the uncertainty of each pixel and utilizes this information to guide the fusion process, which allows the network to adjust the relative contribution of each branch according to the inputs' distribution patterns, as illustrated in \cref{fig:weight}.
%The interaction between these modules makes our method achieve a more efficient and robust completion performance when dealing with sparse and non-uniform inputs. 
%More experiments and results can be found in \cref{sec:Exp}.

In light of the observed variations in focus among local patterns and global semantics across different depth point distributions, our key point is how to dynamically adjust the strength of both local and global features during the depth completion process in scenarios involving depth points with sparsity changes and non-uniform distribution. We propel forward by introducing a novel depth completion network framework named SparseDC to tackle this challenge. 
% which could dynamically adjust the fusion process of local and global features to enhance the performance in scenarios involving depth points with sparsity changes and non-uniform distribution. 
Specifically, to solve the problem of feature instability\cite{woo2023convnext,graham2017submanifold,spconv2022,Sparsitycnn} caused by high variability of depths, we introduce \textit{Sparse Feature Filling Module} that uses immutable image features to fill the varying depth features, thereby improving the ability of network for generalizing to various spatial distributions of depth points. Then, we adopt a two-branch feature extraction structure, where one branch focuses on extracting the local scale information provided by sparse depth points, and the other is more focused on capturing global information to model the scene semantics. After that, the fusion of the extracted features plays a crucial role in SparseDC. Unlike some implicit fusion methods\cite{youmin_completionformer_2023,wang2023lrru}, which depends on the distribution witnessed during training, we design an \textit{Uncertainty-Guided Feature Fusion Module(UFFM)} to dynamically fuse extracted features explicitly. The UFFM uses sparse depths to estimate and correct the uncertainty of each pixel and utilizes this information to guide the fusion process, enabling the network to adjust the relative contribution of each branch based on the distribution patterns of the inputs.

Our proposed method exhibits significant robustness improvement with better efficiency when dealing with sparse and non-uniform depths. We conduct a comprehensive experimental evaluation of our approach on NYU Depth\cite{nyu}, KITTI DC\cite{kitti} and SUN RGB-D\cite{song2015sun}. More experiments and results can be found in \cref{sec:Exp}.


% Some researchers also introduce both the local features and global context information into the depth completion task\cite{youmin_completionformer_2023,wang2023lrru} like us. However, they still perform poorly when facing uneven input, as shown in the Figure. The main reason is that these fuse strategies are implicit, for example, CompletionFormer\cite{youmin_completionformer_2023} stacks convolution layers and attention layers to fuse the local and global information without considering the spatial distribution of input. These distribution-independent fusion strategies make the results inferred by the network depend on patterns seen during training. Therefore, our key idea is to design a distribution-related explicit feature fusion strategy. Specifically, we design an \textit{Uncertainty-Guided Feature Fusion Module(UFFM)}, which uses uneven input to estimate and correct the uncertainty of pixels, and then uses the estimated uncertainty to guide the fusion of global and local information.

% Another challenge comes from convolutional layers. There are some studies have proved that convolutional layers are prone to feature collapse when dealing with highly variable sparsity inputs\cite{woo2023convnext,graham2017submanifold,spconv2022,Sparsitycnn}, which can seriously decrease the performance of the approach. Unlike some sparse convolution-based solutions, our idea comes from the field of depth estimation\cite{bhat2023zoedepth,yuan2022newcrfs,li2023depthformer}, which has demonstrated that deep learning can establish a reasonable mapping between image and depth. So, in this paper, we design a \textit{Sparse Feature Filling Module(SFFM)} to fill stable image features toward invalid depth points to overcome feature instability, improving performance when facing uneven inputs.

% The whole framework of SparseDC is illustrated in Figure *. SparseDC has several key elements: Firstly, we adopt a two-branch feature extraction structure, where one branch focuses on extracting the local scale information provided by sparse depth points, and the other is more focused on capturing global information to model the scene semantics. Secondly, to deal with the uneven input, we design an \textit{Uncertainty Guided Feature Fusion Module}, which dynamically adjusts the overall contribution of each branch through the estimated local uncertainty, making the feature weight distribution suitable for the input distribution. Finally, uneven input will cause feature fluctuations, making it difficult for convolution-based methods to generalize to various spatial distributions of depth points. So, we design a \textit{Sparse Feature Filling Module} to fill stable image features toward invalid depth points to overcome feature instability. 
% unlike SpAgNet\cite{SpAgnet}, we still consider the effective combination of RGB and depth during the encoding, and we design a Sparse Feature Filling Module to fill stable image features toward invalid depth points to overcome feature instability. Secondly, our network  Finally, we design an uncertainty-driven feature fusion strategy, which dynamically adjusts the overall contribution of each branch through the estimated uncertainty and regress to reliable depth maps. 
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/overview_v2.pdf}
    \caption{\textbf{SparseDC Architecture.} Given a sparse depth map and an image, we obtain a stable initial feature $\BO F$ using SFFM. Then, we adopt a two-branch feature extractor to get multi-scale features. After that, the extracted features and sparse depth map are fed to UFFM to obtain the initial depth and estimated uncertainty. Finally, a non-local propagation network\cite{vedaldi_non-local_2020} is exploited for final refinement.}
    \label{fig:overview}
    % \vspace{-1em}
\end{figure*}
Overall, our contributions can be summarized as follows:

\begin{itemize}
    \item We analyze the limitations of mainstream methods when dealing with sparse and non-uniform inputs and propose a novel depth completion framework called SparseDC to tackle this. It consists of several modules that dynamically leverage the complementary strengths of local details and global semantics for robust depth completion.
    \item We access the performance between ours and state-of-the-art methods on some simulated and real challenging cases using indoor\cite{nyu,song2015sun} and outdoor datasets\cite{kitti}. Extensive experiments show the robustness of SparseDC when dealing with sparse and non-uniform depths. 
\end{itemize}


==> sec/intro_bk.tex <==
\section{Introduction}
\label{sec:intro}
% 加引用
Acquiring dense and accurate depth is crucial in various fields, such as autonomous driving\cite{yurtsever2020survey,maurer2016autonomous}, 3D reconstruction\cite{geiger2011stereoscan,long2022pc2,pan2016dense}, scene understanding\cite{cordts2016cityscapes,li2009towards}, AR VR,\cite{yuen2011augmented,park2019literature}. Although the commonly used depth sensors, such as Microsoft Kinect\cite{zhang2012microsoft}, Intel RealSense\cite{keselman2017intel}, LIDAR\cite{atanacio2011lidar}, can obtain depth within their effective field of view, it is still a great challenge to obtain dense depth maps due to environment, equipment, and cost limitations. In recent years, depth completion, serving as a cost-effective means to achieve dense pixel-wise depth, has become a long-standing research endeavor that has captivated the attention of many researchers.

Depth completion aims to recover dense pixel-wise depths from sparse depth maps captured by sensors. In its early stages, previous depth completion methods heavily relied on prior scene knowledge, employing various planar assumptions to interpolate the sparse depth image. In recent years, with the rapid advancements in deep learning, learning-based approaches have emerged as more competitive alternatives, gradually dominating this field. As a pioneering work based on deep learning, Uhrig et al. proposed Sparsity Invariant CNN\cite{Sparsitycnn}, which directly maps sparse depths to dense depth maps using sparse convolution. To push the envelope of depth completion, recent methods focused on stacking complex network architectures and designing sophisticated training strategies, achieving impressive performance on benchmark datasets.
In contrast to the fixed distribution of the benchmark dataset(e.g., NYU Depth with 500 points, Kitti with 64 lines), the inputs in real scenarios are non-uniform and sparser. For example, researchers often employ depth sensors with lower resolutions (Velodyne HDL-16E LiDAR, VCSEL ToF sensors) in real cases to mitigate costs. In addition, environmental factors easily influence sensors, such as high-reflectivity objects and multipath effects resulting in uneven distribution of effective depth points. \textit{\textbf{Regrettably, existing state-of-the-art methods primarily focus on sparse-to-dense conversion without realizing the impact of sparsity changing and non-uniform depth points}}. Consequently, they are difficult to reconstruct the scene structure when the spatial pattern of the input significantly deviates from the distribution observed in the benchmark dataset during training, as illustrated in \cref{fig:teaser}.

To address this challenge, a naive solution is to simulate diverse spatial distributions during training, utilizing a large parameter model to enable the network to adapt to various scenarios. However, designing an effective simulation strategy is highly challenging due to the inherent complexity of real environments. Furthermore, we observed that when dealing with extremely sparse cases, the nature of the task transitions from relying primarily on local details information provided by depth points and texture to relying more heavily on image semantics information for comprehensive scene understanding, which poses limitations of mainstream methods designed only for fixed distribution. To demonstrate this point, we conducted a simple experiment. We selected ResNet-18\cite{resnet} and PvtV2-b1\cite{pvt, pvtv2} as two backbone networks; one is known for its ability to extract local features and capture fine-grained details, and the other focuses on capturing the overall scene context and leveraging global relationships between pixels. We use the NYU Depth V2\cite{nyu} dataset and use the same decoder and the same training strategy (randomly sample depth points between 5 and 500 as input) for both networks. In the testing phase, we randomly sampled 10 times to create a sample of 6,540 images and recorded the final results of the two backbone networks separately. As illustrated in \cref{anaylse}, as the inputs' sparsity increases, the global scene information plays a more important role in depth completion. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/analyse.pdf}
    \caption{\textbf{Pilot study results on NYU Depth V2 dataset}. The first row shows the quantitative analysis. The horizontal axis represents the number of effective depth points used in the test. The vertical axis represents the number of samples that perform better for each branch. The second row is the qualitative results. We visualize the difference in accuracy between different branches, the darker colors indicating more accurate depth predicted by PvtV2-b1.}
    \label{anaylse}
\end{figure}

Based on this observation, we propose a novel depth completion network framework named SparseDC. The key idea behind SparseDC is to \textit{\textbf{effectively leverage the complementary strengths of local details and global semantics to improve the robustness of depth completion in the presence of varying sparsity and non-uniform inputs}}. The whole framework of SparseDC is illustrated in \cref{fig:overview}.  Firstly, we adopt a two-branch feature extraction structure, thus allowing the model to comprehend the holistic scene context while modeling intricate local scale details. Then, some studies proved that uneven input would cause feature fluctuations\cite{woo2023convnext,graham2017submanifold,spconv2022,Sparsitycnn}, making it difficult for our feature extractor to generalize to various spatial distributions of depth points. So, we design a \textit{Sparse Feature Filling Module} that uses immutable image features to fill the varying depth features, thereby improving the stability of the features extracted by different branches. Finally, the fusion of the extracted features plays a crucial role in SparseDC. To tackle this, we introduce an \textit{Uncertainty-Guided Feature Fusion Module(UFFM)}. The UFFM estimates the uncertainty of each pixel and utilizes this information to guide the fusion process, which allows the network to adjust the relative contribution of each branch according to the inputs' distribution patterns, as illustrated in \cref{fig:weight}.
The interaction between these modules makes our method achieve a more efficient and robust completion performance when dealing with sparsity changing and non-uniform inputs. 
More experiments and results can be found in \cref{sec:Exp}.
% Some researchers also introduce both the local features and global context information into the depth completion task\cite{youmin_completionformer_2023,wang2023lrru} like us. However, they still perform poorly when facing uneven input, as shown in the Figure. The main reason is that these fuse strategies are implicit, for example, CompletionFormer\cite{youmin_completionformer_2023} stacks convolution layers and attention layers to fuse the local and global information without considering the spatial distribution of input. These distribution-independent fusion strategies make the results inferred by the network depend on patterns seen during training. Therefore, our key idea is to design a distribution-related explicit feature fusion strategy. Specifically, we design an \textit{Uncertainty-Guided Feature Fusion Module(UFFM)}, which uses uneven input to estimate and correct the uncertainty of pixels, and then uses the estimated uncertainty to guide the fusion of global and local information.

% Another challenge comes from convolutional layers. There are some studies have proved that convolutional layers are prone to feature collapse when dealing with highly variable sparsity inputs\cite{woo2023convnext,graham2017submanifold,spconv2022,Sparsitycnn}, which can seriously decrease the performance of the approach. Unlike some sparse convolution-based solutions, our idea comes from the field of depth estimation\cite{bhat2023zoedepth,yuan2022newcrfs,li2023depthformer}, which has demonstrated that deep learning can establish a reasonable mapping between image and depth. So, in this paper, we design a \textit{Sparse Feature Filling Module(SFFM)} to fill stable image features toward invalid depth points to overcome feature instability, improving performance when facing uneven inputs.

% The whole framework of SparseDC is illustrated in Figure *. SparseDC has several key elements: Firstly, we adopt a two-branch feature extraction structure, where one branch focuses on extracting the local scale information provided by sparse depth points, and the other is more focused on capturing global information to model the scene semantics. Secondly, to deal with the uneven input, we design an \textit{Uncertainty Guided Feature Fusion Module}, which dynamically adjusts the overall contribution of each branch through the estimated local uncertainty, making the feature weight distribution suitable for the input distribution. Finally, uneven input will cause feature fluctuations, making it difficult for convolution-based methods to generalize to various spatial distributions of depth points. So, we design a \textit{Sparse Feature Filling Module} to fill stable image features toward invalid depth points to overcome feature instability. 
% unlike SpAgNet\cite{SpAgnet}, we still consider the effective combination of RGB and depth during the encoding, and we design a Sparse Feature Filling Module to fill stable image features toward invalid depth points to overcome feature instability. Secondly, our network  Finally, we design an uncertainty-driven feature fusion strategy, which dynamically adjusts the overall contribution of each branch through the estimated uncertainty and regress to reliable depth maps. 

Overall, our contributions can be summarized as follows:

\begin{itemize}
    \item We demonstrate the limitations of mainstream methods in dealing with varying sparsity and non-uniform inputs.
    \item We propose a novel depth completion framework named SparseDC, consisting of several well-designed modules that effectively leverage the complementary strengths of local details and global semantics for robust depth completion.
    \item Extensive experiments show that our method performs better when dealing with sparsity changing and non-uniform input on indoor and outdoor datasets.
\end{itemize}
